Data and Analysis Preservation, Recasting, and Reinterpretation

We make the case for the systematic, reliable preservation of event-wise data, derived data products, and executable analysis code. This preservation enables the analyses' long-term future reuse, in order to maximise the scientific impact of publicly funded particle-physics experiments. We cover the needs of both the experimental and theoretical particle physics communities, and outline the goals and benefits that are uniquely enabled by analysis recasting and reinterpretation. We also discuss technical challenges and infrastructure needs, as well as sociological challenges and changes, and give summary recommendations to the particle-physics community.

==> Makefile <==
FILENAME = ms

date = $(shell date +%Y-%m-%d)
output_file = draft_$(date).pdf

figure_src = $(wildcard figures/*.tex figures/*/*.tex)
figure_list = $(figure_src:.tex=.pdf)

LATEX = pdf 

BIBTEX = bibtex

default: document copy_draft

all: default

figures: $(figure_list)

figures/%.pdf: figures/%.tex
	latexmk -$(LATEX) -interaction=nonstopmode -halt-on-error $(basename $@)
	mv $(notdir $(basename $@)).pdf $(basename $@).pdf
	rm $(notdir $(basename $@)).*

text:
	latexmk -$(LATEX) -logfilewarnings -halt-on-error -shell-escape $(FILENAME)

document: figures text

copy_draft:
	rsync $(FILENAME).pdf $(output_file)

clean:
	rm -f *.aux *.bbl *.blg *.dvi *.idx *.lof *.log *.lot *.toc \
		*.xdy *.nav *.out *.snm *.vrb *.mp \
		*.synctex.gz *.brf *.fls *.fdb_latexmk \
		*.glg *.gls *.glo *.ist *.alg *.acr *.acn \
		mainNotes.bib

clean_figures:
	rm -f $(figure_list)

clean_drafts:
	rm -f draft_*.pdf

realclean: clean clean_figures
	rm -f *.ps *.pdf

lint:
	grep -E --color=always -r -i --include=\*.tex --include=\*.bib "(\b[a-zA-Z]+) \1\b" || true

final:
	if [ -f *.aux ]; then \
		$(MAKE) clean; \
	fi
	$(MAKE) figures
	$(MAKE) abstract
	$(MAKE) text
	$(MAKE) clean
	$(MAKE) lint

arXiv: realclean document
	mkdir submit_to_arXiv
	cp $(FILENAME).tex submit_to_arXiv
	if [ -f $(FILENAME).bbl ]; then cp $(FILENAME).bbl submit_to_arXiv/ms.bbl; fi
	cp Makefile submit_to_arXiv

	if [ -d src ]; then cp -r src submit_to_arXiv; fi
	if [ -d latex ]; then cp -r latex submit_to_arXiv; fi
	if [ -d figures ]; then cp -r figures submit_to_arXiv; fi
	if [ -f *.sty ]; then cp *.sty submit_to_arXiv; fi
	
	if [ -f 00README.XXX ]; then cp 00README.XXX submit_to_arXiv; fi

	
	if [ -f $(FILENAME).gls ]; then cp $(FILENAME).gls submit_to_arXiv/ms.gls; fi

	mv submit_to_arXiv/$(FILENAME).tex submit_to_arXiv/ms.tex

	
	
	sed -i.bak '/^ *

	
	
	
	
	

	find submit_to_arXiv/ -name "*.bak" -type f -delete

	
	find submit_to_arXiv/ -name "*.bib" -type f -delete

	tar -zcvf submit_to_arXiv.tar.gz submit_to_arXiv/
	rm -rf submit_to_arXiv
	$(MAKE) realclean

clean_arXiv:
	if [ -f submit_to_arXiv.tar.gz ];then \
		rm submit_to_arXiv.tar.gz; \
	fi

deep_clean: realclean clean_arXiv
	rm -rf submit_to_arXiv

